MultiDepth: Single-Image Depth Estimation via Multi-Task Regression and Classification

We introduce MultiDepth, a novel training strategy and convolutional neural network (CNN) architecture that allows approaching single-image depth estimation (SIDE) as a multi-task problem. SIDE is an important part of road scene understanding. It, thus, plays a vital role in advanced driver assistance systems and autonomous vehicles. Best results for the SIDE task so far have been achieved using deep CNNs. However, optimization of regression problems, such as estimating depth, is still a challenging task. For the related tasks of image classification and semantic segmentation, numerous CNN-based methods with robust training behavior have been proposed. Hence, in order to overcome the notorious instability and slow convergence of depth value regression during training, MultiDepth makes use of depth interval classification as an auxiliary task. The auxiliary task can be disabled at test-time to predict continuous depth values using the main regression branch more efficiently. We applied MultiDepth to road scenes and present results on the KITTI depth prediction dataset. In experiments, we were able to show that end-to-end multi-task learning with both, regression and classification, is able to considerably improve training and yield more accurate results.

==> acronyms.tex <==
%
\newacronym{fps}{FPS}{frames per second}
\newacronym{gta}{GTA~V}{Grand Theft Auto V}
\newacronym{side}{SIDE}{single-image depth estimation}
\newacronym{fcn}{FCN}{fully-convolutional network}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{miou}{MIoU}{mean intersection over union}
\newacronym{relu}{ReLU}{rectified linear unit}
\newacronym{aspp}{ASPP}{atrous spatial pyramid pooling}
\newacronym{resnet}{ResNet}{residual network}
\newacronym{rmsctd}{RMSCTD}{root mean squared cyclic time difference}
\newacronym{sfm}{SfM}{structure from motion}
\newacronym{slam}{SLAM}{simultaneous localization and mapping}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{dorn}{DORN}{deep ordinal regression network}
\newacronym{rmse}{RMSE}{root mean squared error}
\newacronym{silog}{SILog}{scale invariant logarithmic error}
\newacronym{lidar}{LiDAR}{light detection and ranging}
\newacronym[shortplural=ADAS]{adas}{ADAS}{advanced driver assistance system}
%
\newglossaryentry{rsu}{name=road scene understanding, description={}}
\newglossaryentry{cv}{name=computer vision, description={}}
\newglossaryentry{av}{name=autonomous vehicle, description={}}
\newglossaryentry{ad}{name=autonomous driving, description={}}
\newglossaryentry{mt}{name=multi-task, description={}}
\newglossaryentry{md}{name=MultiDepth, description={}}
\newglossaryentry{si}{name=synthetic images, description={}}
\newglossaryentry{ann}{name=artificial neural network, description={}}
\newglossaryentry{cg}{name=computer graphics, description={}}
\newglossaryentry{std}{name=synthetic training data, description={}}
\newglossaryentry{aux}{name=auxiliary task, description={}}
\newglossaryentry{main}{name=main task, description={}}
\newglossaryentry{semseg}{name=semantic segmentation, description={}}
\newglossaryentry{ir}{name=image recognition, description={}}
\newglossaryentry{ac}{name=atrous convolution, description={}}
\newglossaryentry{conv}{name=convolutional, description={}}
\newglossaryentry{max}{name=max pooling, description={}}
\newglossaryentry{fc}{name=fully connected, description={}}
\newglossaryentry{softmax}{name=softmax, description={}}
\newglossaryentry{ce}{name=cross entropy, description={}}
\newglossaryentry{batch}{name=mini batch, description={}}
\newglossaryentry{ow}{name=open world, description={}}
\newglossaryentry{od}{name=object detection, description={}}
\newglossaryentry{sctd}{name=squared cyclic time difference, description={}}
\newglossaryentry{loss}{name=loss function, description={}}
\newglossaryentry{ic}{name=image classification, description={}}
\newglossaryentry{at}{name=atomic task, description={}}
\newglossaryentry{vb}{name=vision-based, description={}}
\newglossaryentry{e-d}{name=encoder-decoder, description={}}
\newglossaryentry{psp}{name=PSPNet, description={}}
\newglossaryentry{kitti}{name=KITTI, description={}}
\newglossaryentry{kside}{name=KITTI depth prediction, description={}}
\newglossaryentry{e}{name=encoder, description={}}
\newglossaryentry{d}{name=decoder, description={}}
\newglossaryentry{dataset}{name=synMT, description={}}
\newglossaryentry{pp}{name=pyramid pooling, description={}}
\newglossaryentry{lr}{name=learning rate, description={}}
\newglossaryentry{dl}{name=deep learning, description={}}

